IMU-HOI: A Symbiotic Framework for Coherent Human-Object Interaction and Motion Capture via Contact-Conscious Inertial Fusion

Capturing full-body human motion with object interactions is crucial for AR/VR and robotics applications, yet it remains challenging for conventional vision-based methods due to occlusions and constrained capture volumes. Inertial measurement units (IMUs) offer a compelling alternative without line-of-sight requirements, but existing IMU-based motion capture assumes an isolated human and ignores object contacts and dynamics. To bridge this gap, we present IMU-HOI, a novel framework that jointly recovers full-body human pose and 6-DoF object trajectory from sparse IMUs on the body and object, explicitly modeling human-object interaction. Our approach first infers probabilistic hand-object contacts directly from IMU streams and uses them as a high-level signal to route between kinematic and inertial reasoning. These contact cues drive a three-stage fusion pipeline that refines human pose and root translation, and fuses hand-based forward kinematics with object-IMU integration for object motion, yielding coherent, drift-resilient trajectories for both human and object. Experiments on challenging human-object interaction scenarios demonstrate substantial accuracy gains over prior inertial motion capture methods. Moreover, IMU-HOI can be plugged into existing sparse-IMU mocap backbones with minimal changes, effectively extending the scope of purely inertial motion capture from isolated humans to full human-object interaction and joint motion estimation.

==> sec/3_method_old.tex <==
\section{Method}

\begin{figure*}[t]
    \centering
    % 调整宽度比例 0.95\linewidth 或 1.0\linewidth 都可以
    \includegraphics[width=0.75\linewidth]{figs/pipeline.pdf}
    \vspace{-0.5em}
    \caption{
        The pipeline of \textbf{I’m-HOI}. Assuming video and inertial measurements input,
        our approach consists of a general interaction motion inference module (Sec.~3.1)
        and a category-specific interaction diffusion filter (Sec.~3.2)
        to capture challenging interaction motions.
    }
    \label{fig:pipeline}
    \vspace{-1em} % 调整与正文间距
\end{figure*}

We address human--object interaction (HOI) estimation from sparse inertial sensing by decomposing the problem into (i) estimating short-horizon motion cues and hand contacts, (ii) estimating human pose and root translation, and (iii) reconstructing the object translation through a contact-conditioned, multi-branch fusion. The design treats contact as a first-class probabilistic signal that steers kinematic or inertial reasoning at each instant, yielding an interpretable and drift-resistant estimator.

\medskip\noindent\textbf{Inputs and notation.}
At time $t$ we observe human IMU $\mathbf{X}^{\text{hum}}_t \!\in \mathbb{R}^{N_{\text{hum}}\times9}$ and an object IMU $\mathbf{X}^{\text{obj}}_t \!\in \mathbb{R}^9$, together with an initial state 
\[
\mathcal{S}_0=\{\mathbf{pose}_0,\ \mathbf{p}_{\mathrm{root}}(0),\ {}^{W}\!R_O(0),\ \mathbf{p}_O(0)\},
\] 
where ${}^{W}\!R_O(t)\in SO(3)$ and $\mathbf{p}_{\mathrm{root}}(t),\mathbf{p}_O(t)\in\mathbb{R}^3$ are the positions of root and objects.

Our pipeline consists of three stages: \textbf{Stage~I} takes $\{\mathbf{X}^{\text{hum}}_{1:T},\mathbf{X}^{\text{obj}}_{1:T},\mathcal{S}_0\}$ and predicts the velocity of the object $\hat{\mathbf v}_O(t)$, the velocities of the hand $\hat{\mathbf v}^{(L)}_H(t),\hat{\mathbf v}^{(R)}_H(t)$, and the probabilities of hand--object contact encoded as 
\[
\boldsymbol{\pi}_t=[p_L(t),p_R(t),1-\max(p_L(t),p_R(t))]. 
\]
\textbf{Stage~II} takes human IMUs and the initial human state and outputs a reduced body pose, full-body joints $\hat{\mathbf{J}}_t\!\in\!\mathbb{R}^{24\times3}$, a root translation trajectory $\hat{\mathbf p}_{\mathrm{root}}(t)$, and wrist positions $\hat{\mathbf p}^{(L)}_H(t),\hat{\mathbf p}^{(R)}_H(t)$ in world coordinates. \textbf{Stage~III} takes the object IMU, ${}^{W}\!R_O(t)$, Stage-I estimates $(\hat{\mathbf v}_O(t),\boldsymbol{\pi}_t)$, and Stage-II wrist trajectories, and produces three object-translation hypotheses $\hat{\mathbf p}^{FK\!-\!L}_O(t)$, $\hat{\mathbf p}^{FK\!-\!R}_O(t)$ and $\hat{\mathbf p}^{IMU}_O(t)$, which are fused with contact-gated weights $w_{t,k}$ into the final trajectory of the object 
\[
\hat{\mathbf p}_O(t)=\hspace{-1em}\sum_{k\in\{L,R,IMU\}} \hspace{-1em}w_{t,k}\,\hat{\mathbf p}^{(k)}_O(t). 
\]

Unless otherwise stated, our experiments report metrics on human pose $\hat{\mathbf{J}}_t$, root translation $\hat{\mathbf p}_{\mathrm{root}}(t)$ and object translation $\hat{\mathbf p}_O(t)$.

\subsection{Stage~I: Velocity--Contact estimation (all IMUs).}

We cast the momentary \emph{contact state} as a categorical distribution over $\{L,R,0\}$ (left hand, right hand, and no-contact). We parameterize
\[
\boldsymbol{\pi}_t = \big[p_L(t),\ p_R(t),\ 1-\max(p_L(t),p_R(t))\big]\in \Delta^2 ,
\]
which (i) preserves mass when neither hand is in contact, (ii) avoids double counting during transitions or bimanual touches by collapsing the ``shared'' mass into the complement, and (iii) directly maps to the three object-translation sources used later (left-FK, right-FK, IMU). A compact LSTM head produces logits from a window of $\{\text{human IMUs}, \text{object IMU}, \hat{\mathbf v}_O, \hat{\mathbf v}_{hands}\}$; we train with \emph{focal cross-entropy}
\[
\mathcal{L}_{\text{hands}}=\sum_t\!\! \sum_{k\in\{L,R,0\}}\!\!\! -\alpha_k (1-q_{t,k})^\gamma\, y_{t,k}\log q_{t,k},
\]
with $\gamma\in[1,2]$ and class weights $\alpha_k$ to handle long no-contact stretches and brief contact spikes. To ensure that $\boldsymbol{\pi}_t$ can act as a \emph{calibrated prior} for fusion, we apply temperature scaling on a held-out split and add a light Kullback--Leibler regularizer during training that discourages over-confident miscalibration.

In parallel, another head regresses \emph{object linear velocity} $\hat{\mathbf v}_O$ from $\{IMU_O,\Delta R_O\}$ using Huber loss, augmented with a short-horizon integral constraint that ties predicted velocity to displacement:
\begin{align*}
\mathcal{L}_{\text{vel}} &= \sum_t \rho\!\big(\hat{\mathbf v}_O(t)-\mathbf v_O(t)\big)\\&+\lambda_{int}\!\!\sum_t\!\Big\|\textstyle\sum_{\tau=t}^{t+\delta}\hat{\mathbf v}_O(\tau)\Delta t-\Delta\mathbf p_O(t\!\to\!t+\delta)\Big\|_1 .
\end{align*}

A differentiable \emph{object-stationarity gate} down-weights both $\|\hat{\mathbf v}_O\|$ and spurious contact logits when the object IMU indicates near-zero motion, reducing false positives in quiescent segments.

%======================= Stage II ======================================

\subsection{Stage-II: Human pose and root translation}
\label{subsec:stage2}

Stage-II estimates a temporally consistent human pose and root translation from human IMUs and the hand velocities provided by Stage-I. The module follows the pipeline in Fig.~\ref{fig:pipeline} (left-bottom) and is implemented as a unified \texttt{HumanPoseModule}.

\medskip\noindent\textbf{Problem setting.}
Let $\mathbf{X}_{1:T}$ denote the sequence of human IMU measurements, where each frame $\mathbf{X}_t$ contains 3D specific force and a 6D orientation representation for all sensors. The goal of Stage-II is to predict: (i) a reduced global body pose, (ii) per-part joint velocities, (iii) per-foot contact probabilities, and (iv) a physically plausible root-translation trajectory that is consistent with both IMU signals and foot--ground contact.

\medskip\noindent\textbf{Baseline: DynaIP-style part-based pose.}
Our pose backbone is based on our previous work Dynamic Inertial Poser (DynaIP)~\cite{zhang2024dynamic}, which demonstrates that decomposing the body into parts significantly stabilizes IMU-based HPE. The body and IMUs are partitioned into three regions (lower limbs, trunk, upper limbs). A lightweight global RNN first summarizes $\mathbf{X}_{1:T}$ into a low-dimensional global context feature per frame. For each region, a dedicated \emph{SubPoser} then takes the region-specific IMUs and the global context as input and outputs (i) local joint velocities and (ii) a reduced set of global joint rotations for the joints within that region. Concatenating the three SubPosers yields a reduced global pose (covering hips, spine, neck, shoulders, etc.) as well as part-wise velocity predictions for lower limbs, trunk, and upper limbs.

To obtain a full 24-joint body, we insert the reduced rotations into a standard SMPL body model, complement them with calibrated sensor orientations for the remaining bones, and apply global-to-local conversion followed by differentiable forward kinematics (FK). This produces world-space joint positions $\hat{\mathbf{J}}_t$, which serve both as the final pose output of Stage-II and as intermediate cues for root translation.

\medskip\noindent\textbf{Baseline: TransPose root translation.}
For root translation, we build on the TransPose framework~\cite{yi2021transpose}, which estimates global translation from six IMUs via two complementary branches. The \textbf{B1} branch infers which foot is in contact and converts the contacting foot’s FK trajectory into a root-motion proxy; the \textbf{B2} branch regresses local root velocity from joint positions and IMUs using an RNN. A scalar contact confidence derived from foot-contact logits is used to blend the two root-velocity hypotheses, and the fused velocity is integrated over time with simple floor constraints to avoid penetration. Conceptually, we adopt the same two-branch design and fusion strategy, but change the \emph{inputs} of both branches to better exploit DynaIP’s part-based structure and velocity outputs.

\medskip\noindent\textbf{Our part-based human pose and translation module.}
Our Stage-II module couples the DynaIP-style SubPosers with a TransPose-style translation head through two key modifications.

\smallskip\noindent
\textbf{(1) Trunk-velocity driven B2 branch.}
Instead of feeding all joint positions into the B2 RNN as in TransPose, we construct a compact \emph{trunk-velocity} descriptor from the DynaIP outputs. Specifically, from the FK joint positions $\hat{\mathbf{J}}_t$ we select the trunk subset (hips, spine1~3, neck and head) and compute finite-difference velocities to obtain a vector of trunk velocities. The B2 RNN then takes as input this trunk-velocity vector, along with IMUs around the root and head and the global context feature, and predicts the local root velocity, which is finally rotated into world coordinates by the root IMU orientation.

This design is motivated by three observations:
(i) trunk joints are much more stable than extremities such as hands and feet and are strongly correlated with the motion of the body center, yielding a cleaner and more informative signal for root-velocity estimation;
(ii) DynaIP already provides a modular decomposition into lower limbs, trunk, and upper limbs, so trunk-related pose and velocity features are estimated independently which can be extracted \emph{for free} without adding new parameters or supervision;
(iii) providing velocities instead of positions as inputs makes it more temporally smooth and closer to the B2 prediction target (root velocity), eliminating the need for implicit differentiation inside the network and reducing drift.

\smallskip\noindent
\textbf{(2) Lower-limb velocity driven B1 branch.}
For the B1 branch, TransPose uses leaf-joint positions (feet) and IMUs to estimate foot--ground contact and derive a contact-driven root-motion proxy. In our design, we reuse the \emph{lower-limb velocities} predicted by the DynaIP SubPoser. We extract the velocities of both feet and the root from the lower-limb velocity vector and feed them, together with foot IMUs and the global context, into the B1 RNN. The RNN outputs foot-contact logits, from which we derive contact probabilities for the left and right foot. The contact-driven root-velocity hypothesis is then obtained by following the TransPose strategy: we select the more likely contacting foot and map its FK velocity to a root velocity, adding a small learned gravity bias.

Using velocities instead of positions has two advantages in this branch:
(i) foot contact is more directly characterized by near-zero velocities than by positions, leading to sharper and more reliable contact detection, especially in the presence of drift;
(ii) DynaIP already estimates foot velocities as intermediate outputs, so our B1 branch can simply reuse these signals without additional layers or supervision.

\medskip\noindent\textbf{Contact-aware fusion, floor handling, and outputs.}
Given the world-space root velocity from B2 and the contact-driven velocity from B1, we compute a scalar contact confidence from the maximum foot-contact probability. This confidence is transformed into a fusion weight $w_t \in [0,1]$ and used to blend the two hypotheses in a convex combination, as in TransPose. When contact is confident, B1 dominates and enforces stable motion around the supporting foot; when contact is uncertain, B2 provides a smoother, IMU-driven estimate.

To avoid floor penetration, we monitor the minimum vertical foot height over time and maintain a cumulative non-negative correction on the vertical component of the fused root velocity whenever the feet would move below a known floor level. Integrating the corrected velocities over time yields the root translation trajectory. Adding this translation back to the FK joint positions provides world-space joint trajectories, in particular the world-space wrist positions that are forwarded to Stage-III for human--object interaction reasoning.

\medskip\noindent\textbf{Training.}
Stage-II is supervised using standard losses on joint rotations and positions, per-part velocities, foot-contact probabilities, root velocity, and integrated root translation. Importantly, our modifications do not require any additional labels: all new inputs to B1 and B2 (trunk and lower-limb velocities) are derived from the DynaIP-style SubPosers, and the overall training protocol remains consistent with the original DynaIP and TransPose settings.


%=====================================================================
\subsection{Stage~III: Object translation via contact-gated fusion (unified three-branch).}
Stage~III estimates the global object translation by fusing \emph{two kinematic (FK) branches}, conditioned on the left/right hands, with an \emph{IMU-driven branch}. 
The design is built around a simple, yet very useful, simplification of hand--object interaction:

\medskip\noindent\textbf{Quasi-rigid contact assumption.}
Once a hand establishes contact with the object, we assume that the corresponding contact point on the object \emph{remains fixed in the object coordinate frame} for the entire interaction segment. 
Let ${}^W\!R_O(t)$ denote the object IMU orientation, ${}^W\!\mathbf{p}^{(s)}_H(t)$ the position of hand $s\in\{L,R\}$ in world coordinates, and ${}^W\!\mathbf{p}_O(t)$ the object IMU position. 
Under the fixed-contact assumption, the vector from the contact point to the object IMU, expressed in the object frame, is constant:
\[
{}^O\!\mathbf{d}^{(s)} \;=\; {}^W\!R_O(t)^\top\Bigl({}^W\!\mathbf{p}_O(t) - {}^W\!\mathbf{p}^{(s)}_H(t)\Bigr) ,
\]
so that
\[
{}^W\!\mathbf{p}_O(t) \;=\; {}^W\!\mathbf{p}^{(s)}_H(t) \;+\; {}^W\!R_O(t)\,{}^O\!\mathbf{d}^{(s)} .
\]
In other words, once the contact point is known, the object position can be fully determined from the hand position and object IMU pose by a simple geometric relation.

In our setting, we \emph{do not} have access to the object mesh, so we cannot refine the contact point by enforcing mesh-based geometric constraints. 
Consequently, estimating ${}^O\!\mathbf{d}^{(s)}$ becomes challenging and highly dependent on (i) the accuracy of the human pose estimation for the hands and (ii) the reliability of the hand--object contact labels. 
Stage~III is designed to \emph{learn} this contact offset from data, while leveraging both kinematics and inertial cues.

\medskip\noindent\textbf{Why FK--IMU fusion?}
We deliberately choose to combine FK and IMU cues instead of relying on a single source.

\begin{itemize}
    \item \textbf{IMU-only.} 
    Integrating object accelerations from the IMU provides a direct and conceptually simple path to translation. 
    Over short time windows, this integration is reasonably accurate and drift is limited. 
    However, sensor noise, bias, and integration errors inevitably accumulate, causing \emph{large long-term drift} in the estimated trajectory.
    \item \textbf{FK-only.}
    FK leverages the explicit interaction structure: as long as the hand stays in contact and the fixed-contact assumption holds, the induced object trajectory does \emph{not} drift over time and remains consistent with the human motion.
    On the downside, FK is very sensitive to errors in contact labels and hand positions; an incorrect contact point may lie off the true mesh, leading to a biased translation estimate. 
    Moreover, pure FK cannot model relative sliding between the hand and the object during interaction.
\end{itemize}

Therefore, we adopt a \emph{fusion} strategy: FK is used to regularize and reduce IMU drift when contact is confident, while the IMU branch provides complementary motion information in regimes where FK is locally unreliable (e.g., at contact on/off, transient sliding, or ambiguous contacts).We also perform an ablation study on the fusion strategy in Sec.~\ref{subsec:ablation}, comparing IMU-only, FK-only, and fused variants to validate our theoretical analysis.

% ---------------- Table 1 (equal column widths) ----------------
% uniform column widths: tweak \cw if needed
\newcommand{\cw}{0.88cm}                 % each metric column width
\newcommand{\mw}{1.5cm}                  % Methods column width
\newcolumntype{C}{>{\centering\arraybackslash}m{\cw}}
\newcolumntype{L}{>{\raggedright\arraybackslash}m{\mw}}
\begin{table*}[t]
\centering
\caption{Comparison on three HOI datasets. Numbers are lower-is-better. Best in \textbf{bold}.}
\label{tab:sota_without_root}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.06}
\scriptsize
\resizebox{\linewidth}{!}{%
\begin{tabular}{L*{15}{C}}
\toprule
& \multicolumn{5}{c}{OMOMO} 
& \multicolumn{5}{c}{$IMHD^{2}$} 
& \multicolumn{5}{c}{BEHAVE} \\
\cmidrule(lr){2-6}\cmidrule(lr){7-11}\cmidrule(lr){12-16}
\textbf{Methods} 
& Obj Err  & HOI Err  & Ang Err  & Pos Err  & Jitter
& Obj Err  & HOI Err  & Ang Err  & Pos Err  & Jitter
& Obj Err  & HOI Err  & Ang Err  & Pos Err  & Jitter \\
\midrule
DIP* 
& 25.84 & 26.79 & 3.05 & 3.34 & 2.74
& 90.37 & 93.09 & 7.36 & 8.97 & 9.57
& 38.91 & 39.31 & 4.79 & 4.70 & 7.04 \\
TIP* 
& 44.41 & 48.01 & 5.48 & 8.55 & 5.77
& 92.75 & 106.74 & 10.84 & 49.23 & 66.88
& 26.43 & 30.24 & 7.86 & 11.97 & 8.47 \\
Transpose* 
& 32.54 & 32.73 & 4.48 & 3.15 & \textbf{2.47}
& 90.37 & 90.61 & 7.76 & 5.27 & 9.57
& 40.39 & 40.40 & 6.71 & 3.71 & 8.58 \\
GlobalPose* 
& 39.34 & 39.51 & 4.13 & 3.69 & 4.04
& 101.27 & 102.03 & 6.61 & 8.31 & \textbf{8.17}
& 40.14 & 40.21 & 6.00 & 4.73 & \textbf{6.88} \\
\textbf{Ours (Fusion)} 
& \textbf{14.15} & \textbf{14.94} & \textbf{2.84} & \textbf{2.27} & 2.75
& \textbf{49.76} & \textbf{51.09} & \textbf{4.51} & \textbf{3.85} & 10.57
& \textbf{22.26} & \textbf{22.62} & \textbf{4.52} & \textbf{2.72} & 8.20 \\
\bottomrule
\end{tabular}%
}
\vspace{-0.6em}
\end{table*}

% ---------------- Table 2 (equal column widths) ----------------
\renewcommand{\cw}{0.93cm}   % 指标列宽（Table 2 专用）
\renewcommand{\mw}{1.5cm}   % Methods 列宽（Table 2 专用）
\begin{table*}[t]
\centering
\caption{Main comparison with root-translation and jitter. Numbers are lower-is-better. Best in \textbf{bold}.}
\label{tab:sota_with_root}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.05}
\scriptsize
\resizebox{\linewidth}{!}{%
\begin{tabular}{L*{18}{C}}
\toprule
& \multicolumn{5}{c}{OMOMO}
& \multicolumn{5}{c}{$IMHD^{2}$}
& \multicolumn{5}{c}{BEHAVE} \\
\cmidrule(lr){2-6}\cmidrule(lr){7-11}\cmidrule(lr){12-16}
\textbf{Methods}
& Obj Err & HOI Err & Pos Err & Trans Err & Jitter 
& Obj Err & HOI Err & Pos Err & Trans Err & Jitter 
& Obj Err & HOI Err & Pos Err & Trans Err & Jitter  \\
\midrule
Transpose*
& 32.09 & 40.43 & 6.36 & 19.36 & 6.09
& 94.57 & 100.65 & 5.87 & 37.79 & 10.66
& 50.70 & 55.83 & 6.05 & 23.52 & 11.76 \\
GlobalPose*
& 39.31 & 40.35 & 3.67 & \textbf{10.80} & 3.94
& 103.27 & 108.33 & 8.29 & 58.36 & \textbf{8.15}
& 42.38 & 45.47 & 4.71 & 16.05 & \textbf{6.63} \\
\textbf{Ours (Fusion)}
& \textbf{11.31} & \textbf{17.44} & \textbf{2.35} & 11.07 & \textbf{2.77}
& \textbf{43.97} & \textbf{43.39} & \textbf{3.69} & \textbf{18.37} & 10.38
& \textbf{20.90} & \textbf{25.74} & \textbf{2.77} & \textbf{11.14} & 8.19 \\
\bottomrule
\end{tabular}%
}
\vspace{-0.5em}
\end{table*}

%------------------------------------------


\medskip\noindent\textbf{Kinematic FK branches.}
Stage~III maintains two FK branches, one for each hand $s\in\{L,R\}$. 
A small recurrent head consumes hand kinematics and object IMU orientation and predicts an \emph{object-frame ray direction} and a \emph{non-negative reach length}:
\[
{}^{O}\hat{\mathbf u}^{(s)}_t \in \mathbb S^2,\qquad 
\hat{\ell}^{(s)}_t=\mathrm{softplus}(\phi^{(s)}_t)+\varepsilon .
\]
We interpret ${}^{O}\hat{\mathbf u}^{(s)}_t\,\hat{\ell}^{(s)}_t$ as a learnable approximation of the constant offset ${}^O\!\mathbf{d}^{(s)}$ from the hand contact point to the object IMU in the object frame. 
The resulting world-space FK estimate is
\[
\hat{\mathbf p}^{FK\!-\!s}_O(t)=\hat{\mathbf p}^{(s)}_H(t) +\, {}^{W}\!R_O(t)\,{}^{O}\hat{\mathbf u}^{(s)}_t\,\hat{\ell}^{(s)}_t ,
\]
where $\hat{\mathbf p}^{(s)}_H(t)$ comes from Stage-II wrist positions.
Predicting offsets in the \emph{object frame} factors out global rotation, stabilizing learning across viewpoints and grasp orientations.

\medskip\noindent\textbf{Geometric supervision and HOI loss.}
During training, we explicitly supervise both the direction and length of the object-frame offset whenever the object and hand $s$ are annotated as in contact.
Given ground-truth object and hand positions ${}^W\!\mathbf{p}^{\text{gt}}_O(t)$ and ${}^W\!\mathbf{p}^{(s),\text{gt}}_H(t)$, we derive the object-frame offset target
\[
{}^O\!\mathbf{d}^{(s)}_t = {}^{W}\!R_O(t)^\top \Bigl({}^W\!\mathbf{p}^{\text{gt}}_O(t)-{}^W\!\mathbf{p}^{(s),\text{gt}}_H(t)\Bigr) ,
\]
and decompose it into a unit direction and length. 
We use separate regression losses for the predicted length $\hat{\ell}^{(s)}_t$ and direction ${}^{O}\hat{\mathbf u}^{(s)}_t$, together with a \emph{HOI offset loss} on the reconstructed vector:
\[
\mathcal{L}^{(s)}_{\text{HOI}} 
= \big\|{}^{O}\hat{\mathbf u}^{(s)}_t\,\hat{\ell}^{(s)}_t - {}^O\!\mathbf{d}^{(s)}_t \big\|_2 ,
\]
evaluated only on frames where the hand--object contact mask for $s$ is active.
This term directly measures the discrepancy between the predicted and true hand--object offset in the object frame and is the training counterpart of our HOI error metric. 
We also apply mild regularization to encourage ${}^{O}\hat{\mathbf u}^{(s)}_t$ to be unit-length and to smooth $\hat{\ell}^{(s)}_t$ over time, reducing ``rubber-band'' artifacts.

\medskip\noindent\textbf{IMU branch.}
In parallel, an IMU-conditioned head predicts an object position $\hat{\mathbf p}^{IMU}_O(t)$ from the object IMU sequence and Stage-I object velocities, using as inputs $\{IMU_O,\hat{\mathbf v}_O,\Delta R_O, {}^W\!R_O\}$. 
To alleviate long-term drift, we introduce an \emph{integrated velocity anchor}:
\[
\hat{\mathbf p}^{IMU}_O(t)= \hat{\mathbf p}^{IMU\text{-net}}_O(t) 
\;+\; \eta\!\sum_{\tau\le t}\hat{\mathbf v}_O(\tau)\Delta t ,
\]
so that the network learns a residual correction $\hat{\mathbf p}^{IMU\text{-net}}_O(t)$ around the integrated trajectory rather than the entire translation. 
This branch is supervised by an object-translation loss
\[
\mathcal{L}_{\text{trans}} = 
\big\|\hat{\mathbf p}^{IMU}_O(t)-{}^W\!\mathbf{p}^{\text{gt}}_O(t)\big\|_2^2 ,
\]
evaluated under an object-visibility mask.

\medskip\noindent\textbf{Gated fusion.}
The final object trajectory is obtained via a contact-aware fusion of the two FK branches and the IMU branch. 
Let $g(\cdot)$ be a causal LSTM that observes $\{IMU_O,\hat{\mathbf v}_O,\Delta R_O\}$ (and optionally hand kinematics) and outputs fusion logits $\mathbf z_t\in\mathbb{R}^3$. 
From Stage-I contact heads we derive a simple prior $\boldsymbol{\pi}_t$ over ``left contact'', ``right contact'', and ``no-contact''. 
The fusion weights are computed as
\[
\mathbf w_t=\mathrm{softmax}\!\Big(\tfrac{1}{\tau}\big[\mathbf z_t+\beta\,\log \boldsymbol{\pi}_t\big]\Big), 
\]
and the fused object position is
\[
\hat{\mathbf p}_O(t)=\sum_{k\in\{L,R,IMU\}} w_{t,k}\,\hat{\mathbf p}^{(k)}_O(t),
\]
where $\hat{\mathbf p}^{(L)}_O(t)=\hat{\mathbf p}^{FK\!-\!L}_O(t)$, 
$\hat{\mathbf p}^{(R)}_O(t)=\hat{\mathbf p}^{FK\!-\!R}_O(t)$, and 
$\hat{\mathbf p}^{(IMU)}_O(t)=\hat{\mathbf p}^{IMU}_O(t)$. 
This \emph{Bayesian-style routing} makes fusion interpretable: confident left-hand contact amplifies the left-FK branch; when no-contact dominates, the IMU branch naturally prevails. 
The temperature $\tau$ controls the sharpness of routing (small $\tau$ yields near one-hot switching, larger $\tau$ yields smoother blending).

\medskip\noindent\textbf{Temporal stability.}
To prevent unstable behavior during handovers and noisy contact predictions, we regularize the fusion weights and lightly smooth the FK trajectories. 
In practice, we penalize rapid changes in $\mathbf w_t$ over time, and apply a single-step ``shock absorber'' that dampens implausible jumps of the FK estimates relative to the previous fused object position while preserving gradients. 
These mechanisms stabilize the fused trajectory in contact transition regions without over-smoothing sharp, physically meaningful corrections.

\medskip\noindent\textbf{Kinematic--inertial consistency and total loss.}
Finally, we enforce finite-difference consistency between the fused position $\hat{\mathbf p}_O(t)$ and Stage-I object velocities (and, when available, object accelerations from the IMU):
\begin{align*}
\mathcal{L}_{\text{cons}}&=\sum_t\!\Big\|\Delta \hat{\mathbf p}_O(t)\,f_{\text{fps}}-\hat{\mathbf v}_O(t)\Big\|_1\\
&\quad+\lambda_a\!\sum_t\!\Big\|\Delta^2 \hat{\mathbf p}_O(t)\,f_{\text{fps}}^2-\hat{\mathbf a}_O(t)\Big\|_1 .
\end{align*}
The first term penalizes discrepancies between the discrete velocity implied by Stage~III positions and the Stage-I velocity estimate; the second term aligns the second-order differences with IMU accelerations, effectively suppressing high-frequency jitter while constraining drift.

Overall, Stage~III learns:
(i) the object-frame ray directions ${}^{O}\hat{\mathbf u}^{(s)}_t$ and lengths $\hat{\ell}^{(s)}_t$ that parametrize the contact offset for each hand,
(ii) the IMU-based residual translation head $\hat{\mathbf p}^{IMU\text{-net}}_O(t)$, and
(iii) the gating LSTM that produces the fusion logits $\mathbf z_t$.
The total loss aggregates object translation regression, velocity/acceleration consistency, contact-geometry losses on direction and length, and the HOI offset losses $\mathcal{L}^{(s)}_{\text{HOI}}$. 
This unified three-branch design allows the model to inherit the drift-free interaction structure of FK while leveraging the short-term accuracy of IMU integration, compensating for the weaknesses of each source through contact-aware fusion.


\subsection{Optimization and training schedule}
We adopt a staged curriculum and freeze earlier modules once trained. \textbf{Stage~I} is first trained in isolation with
\[
\mathcal{L}^{(1)} = \mathcal{L}_{\text{hands}} + \lambda_{\text{vel}}\mathcal{L}_{\text{vel}} + \lambda_{\text{cal}}\mathcal{L}_{\text{cal}},
\]
where $\mathcal{L}_{\text{hands}}$ and $\mathcal{L}_{\text{vel}}$ are the focal-contact and velocity losses defined above, and $\mathcal{L}_{\text{cal}}$ denotes the light calibration regularization (temperature scaling, KL prior and the object-stationarity gate). After convergence, \emph{Stage~I is frozen for all subsequent training}.

\textbf{Stage~II} is then trained on top of the frozen Stage~I. Its loss
\[
\mathcal{L}^{(2)} = \mathcal{L}_{\text{pose}} 
+ \lambda_{\text{root}}\mathcal{L}_{\text{root}} 
+ \lambda_{\text{part}}\mathcal{L}_{\text{vel-part}} 
+ \lambda_{\text{feet}}\mathcal{L}_{\text{feet}}
\]
combines standard supervision on joint rotations/positions ($\mathcal{L}_{\text{pose}}$), root velocity/translation ($\mathcal{L}_{\text{root}}$), per-part velocities ($\mathcal{L}_{\text{vel-part}}$) and feet-contact probabilities ($\mathcal{L}_{\text{feet}}$). This yields stable human pose, root trajectory and wrist positions that are kept fixed when training Stage~III (unless explicitly stated otherwise).

\textbf{Stage~III} is optimized in two phases. In the first phase we \emph{freeze both Stage~I and Stage~II} and train only the object-translation module with
\[
\mathcal{L}^{(3)} = \mathcal{L}_{\text{trans}} 
+ \lambda_{\text{cons}}\mathcal{L}_{\text{cons}}
+ \lambda_{\text{HOI}}\mathcal{L}_{\text{HOI}}
+ \lambda_{\text{smooth}}\mathcal{L}_{\text{smooth}},
\]
where $\mathcal{L}_{\text{trans}}$ is the object position regression (obj\_trans), $\mathcal{L}_{\text{cons}}$ collects the velocity/acceleration consistency terms (obj\_vel\_cons, obj\_acc\_cons), $\mathcal{L}_{\text{HOI}}$ aggregates the length and direction losses and the hand--object offset terms for both hands (lhand/rhand\_lb, lhand/rhand\_obj\_direction, hoi\_error\_l/r), and $\mathcal{L}_{\text{smooth}}$ regularizes the temporal variation of fusion weights and FK outputs. After Stage~III has converged, we \emph{unfreeze Stage~II but keep Stage~I frozen}, and perform a short joint fine-tuning of Stage~II+III with a reduced learning rate and total loss
\[
\mathcal{L}^{(2+3)} = \mathcal{L}^{(2)} + \lambda_{\text{joint}}\mathcal{L}^{(3)},
\]
which slightly adjusts human pose and root translation to better support object translation, while preserving the calibrated contact priors from Stage~I. In all experiments, Stage~I is only updated in its dedicated first stage and remains frozen thereafter.

% \medskip\noindent\textbf{Implementation and inference notes}

% All temporal heads are causal LSTMs (1--2 layers, 128--256 hidden units) with SiLU MLPs; training uses 1-s windows with 50\% overlap, while inference runs fully online. FK rays use $\ell_2$ normalization for $^{O}\hat{\mathbf u}$ and Softplus for $\hat{\ell}$ with $\varepsilon=10^{-3}$. We pick $\tau\in[0.4,1.2]$ and $\tau_p\in[0.8,2.0]$ by validation; $\beta$ is set so that a confident contact (e.g., $p\approx0.9$) contributes a $+\log(0.9/0.1)$-scale boost to the relevant FK logit. At test time, if $p_0$ remains high for a span and the object IMU indicates quiescence, we progressively raise $w_{IMU}$ (bounded by the softmax) and perform a zero-velocity update on the IMU branch to clamp drift. The system outputs $\hat{\mathbf p}_O$ together with diagnostics $\hat{\mathbf v}^{diff}_O=\Delta\hat{\mathbf p}_O\, f_{\text{fps}}$ and $\hat{\mathbf a}^{diff}_O=\Delta^2\hat{\mathbf p}_O\, f_{\text{fps}}^2$, enabling automatic detection of inconsistency spikes that transiently increase $\tau$ for safer blending.



==> sec/4_Experiment_old.tex <==
\section{Experiment}
\label{sec:experiments}

The experimental analysis is structured as follows: (1) Experimental Setup: We detail the datasets, evaluation metrics, and implementation specifics. (2) Comparison with State-of-the-Art: We benchmark our method against existing leading approaches. (3) Ablation Studies: We systematically evaluate the contribution of each proposed module. 
%(4) Further Analysis: Additional discussions and visual examples are included in the supplementary material.

\subsection{Experimental Setup}

\paragraph{Datasets.}
We evaluate on three public HOI datasets that differ in capture modality, object diversity, and sequence duration.

\textbf{OMOMO}~\cite{li2023omghm} This set focuses on full-body manipulation of large objects, with roughly $\sim$10 hours of interactions spanning about 15 object categories. Clips are typically short ($\approx$5\,s) and recorded at 30\,fps, featuring actions such as \emph{lift, carry, push, pull, place}.

\textbf{BEHAVE}~\cite{bhatnagar2022behave} Multi-view RGB-D capture of humans interacting with everyday items; 8 subjects and $\sim$20 object categories with diverse everyday actions (e.g., \emph{sitting on, picking up, carrying, pushing/pulling, placing}). The official frame rate is 30\,fps.

$\mathbf{IMHD^{2}}$~\cite{zhao2024imhoi} Video–inertial HOI benchmark at 60\,fps with 10 object categories and rich interaction verbs (\emph{hold, carry, lift, putdown, push, pull, swing, throw/catch}, etc.). Sequences are typically long (often $\ge$60\,s).

\emph{Preprocessing.}
To match temporal statistics, we downsample $IMHD^{2}$ from 60\,fps to 30\,fps. Because $IMHD^{2}$ and BEHAVE contain many $\ge$60\,s sequences while OMOMO clips are around 5\,s, we randomly crop $IMHD^{2}$/BEHAVE into 5–10\,s windows during training and evaluation for balanced sequence lengths.Unless otherwise stated, we adopt an 80/20 train/test split on each dataset at the \emph{sequence} level.For $IMHD^{2}$/BEHAVE, long clips are cropped into 5–10\,s windows \emph{after} the split to avoid leakage. 

\paragraph{Competing methods.}
We compare against four strong IMU-based HPE baselines:
\emph{DIP}~\cite{huang2018deep}(recurrent network for pose from sparse IMUs),
\emph{TIP}~\cite{jiang2022tip}(transformer-based IMU poser),
\emph{TransPose}~\cite{yi2021transpose}(enhanced temporal modeling for sparse-IMU HPE),
and \emph{GlobalPose}~\cite{globalpose_2025} (sparse-IMU HPE augmented with physics-based global motion estimation).
For a fair HOI comparison, we adopt two variants for each: (i) a dimension-augmented baseline that adds an object-IMU branch and an object-velocity head (integrated to object translation), and (ii) the same backbone used as the human module within our contact-gated fusion pipeline. All methods take six body IMUs and one object IMU as input, and share identical splits and evaluation protocols.

\paragraph{Metrics.}
Following prior work~\cite{yi2021transpose,petrov2023object}, we report the following metrics:
\emph{1) Ang Err} [$^\circ$]: the mean global rotation error of all body joints (in degrees);
\emph{2) Pos Err} [cm]: the mean Euclidean distance of all estimated joints with the root joint (Spine) aligned;
\emph{3) Jitter} [mm/s$^3$]: motion smoothness measured by the average \emph{jerk} (rate of change of acceleration) across all joints, where lower is smoother;
\emph{4) Trans Err} [cm]: the average global translation error of the root joint (Spine);
\emph{5) Obj Trans Err} [cm]: the $\ell_2$ distance between the predicted and ground-truth object mesh centers;
\emph{6) HOI Err} [cm] (ours): a \emph{specially} designed interaction metric that evaluates the accuracy of the \emph{relative} hand–object spatial relationship and is computed only on frames with ground-truth hand–object contact. Let $\mathbf{c}^{gt}_t$ and $\hat{\mathbf{c}}_t$ be the GT and predicted object centers, and $\mathbf{h}^{gt}_t$ and $\hat{\mathbf{h}}_t$ the GT and predicted contact-hand joints; with $\mathcal{C}$ the set of GT contact frames, we define
\[
\text{HOI Err}=\frac{1}{|\mathcal{C}|}\sum_{t\in\mathcal{C}}
\big\|(\hat{\mathbf{h}}_t-\hat{\mathbf{c}}_t)-(\mathbf{h}^{gt}_t-\mathbf{c}^{gt}_t)\big\|_2 ,
\]
which emphasizes the accuracy of the hand–object spatial relationship during interaction.

% ---------------- Fig 2 ----------------
\begin{figure}[t]      % t  = 页顶位置（也可以 hbtp 等视情况）
  \centering
  \includegraphics[width=0.48\linewidth]{figs/root_trans_error_curves_OMOMO.pdf}%
  \hfill
  \includegraphics[width=0.48\linewidth]{figs/root_trans_error_curves_BEHAVE.pdf}%
  \caption{Cumulative distance error vs.\ time for OMOMO (left) and BEHAVE (right).}
  \label{fig:curve_trans_error}
\end{figure}
% --------------------------------

% ---------------- Fig 3 ----------------
\begin{figure*}[t]
    \centering
    % 调整宽度比例 0.95\linewidth 或 1.0\linewidth 都可以
    \includegraphics[width=1.0\linewidth]{figs/table1_vis.pdf}
    \vspace{-1.5em}
    \caption{
        Visualization of motion estimation on four sequences.
    }
    \label{fig:qualitative_compare}
    \vspace{-1em} % 调整与正文间距
\end{figure*}
% ---------------- Fig 3 ----------------
\subsection{Comparison with State-of-the-Art}
%先讲 我们分成了两个训练测试的方式（with/without Translation）
%在讲我们对于这些惯性动捕的工作做了什么操作，让他们能够又物体的估计
We categorize prior HPE methods into two training–evaluation protocols, reflecting the fact that most contemporary approaches do not estimate global/root translation: (i) \emph{w/o root translation} (Table~\ref{tab:sota_without_root}) and (ii) \emph{with root translation} (Table~\ref{tab:sota_with_root}). Under protocol (i), for methods that originally include a translation head, we ablate that component and substitute the root translation with ground truth (GT) to isolate pose quality; the resulting models are re-trained and evaluated on the target datasets for fair comparison. Under protocol (ii), translation-capable baselines are kept intact and trained/evaluated end to end. This setup ensures apples-to-apples comparisons across methods with and without explicit root translation modeling.Curves of cumulative root-translation error are shown in Fig.~\ref{fig:curve_trans_error}. Qualitative comparisons are in Fig.~\ref{fig:qualitative_compare}.


\paragraph{Quantitative Experimental Analysis. }
%最后讲述实验结果，分成（with/without Translation），说明我们的方法具有先进性
We compare our proposed method with the competing methods on the three public human-object interaction datasets. When the root translation estimation is disabled, across all three datasets in Table~\ref{tab:sota_without_root}, our method attains the lowest Obj Err and HOI Err in nearly every case, e.g., on OMOMO (14.15 / 14.94), $IMHD^{2}$ (49.76 / 51.09), and BEHAVE (22.26 / 22.62). \emph{Compared to GlobalPose*}, our method achieves substantial reductions on Obj Err by 25.19 (64.0\%) / 51.51 (50.9\%) / 17.88 (44.5\%) and on HOI Err by 24.57 (62.2\%) / 50.94 (49.9\%) / 17.59 (43.7\%) on OMOMO / $IMHD^{2}$ / BEHAVE, respectively. 
These two metrics directly reflect the fidelity of the estimated object trajectory and human–object relations; the consistent gains indicate that modeling contact and jointly reasoning over human- and object-IMUs is crucial even when root translation is not evaluated.
Beyond interaction-centric scores, our method also achieves state-of-the-art Ang Err and Pos Err across all datasets, e.g., Ang Err 2.84 / 4.51 / 4.52 and Pos Err 2.27 / 3.85 / 2.72 on OMOMO / $IMHD^{2}$ / BEHAVE, respectively.

When root translation is evaluated (Table~\ref{tab:sota_with_root}), our method maintains clear advantages on Obj Err and HOI Err across datasets, while also delivering competitive root-translation accuracy. On OMOMO, our Trans Err is \emph{on par} with GlobalPose*, within 0.27 (2.5\%) of its score; on the smaller $IMHD^{2}$ set we \emph{reduce} Trans Err by 39.99 (68.5\%), and on BEHAVE by 4.91 (30.6\%). This contrast suggests that GlobalPose* benefits strongly from large-scale training, whereas our contact-gated, RNN-based estimator generalizes better with limited data.Notably, under the \emph{with root translation} setting, we focus on position metrics, so Table~\ref{tab:sota_with_root} omits angular pose errors, despite our method maintaining an advantage in these metrics as well.


Figure~\ref{fig:curve_trans_error} plots cumulative root-translation error over time. On BEHAVE our curve stays consistently below both TransPose* and GlobalPose*, and on OMOMO we clearly outperform TransPose* and remain on par with GlobalPose*. 
Beyond accuracy, our model runs \emph{an order of magnitude faster} than GlobalPose*: the latter relies on per-frame physical optimization in its forward pass, whereas our network is a lightweight causal RNN that performs a single feed-forward pass per step, enabling practical deployment.

\paragraph{Qualitative Experimental Analysis.}
%挑选1-2个数据中的3-5条序列，进行可视化展示，从中找到一些我们的优势点
Figure~\ref{fig:qualitative_compare} visualizes results on \textbf{untrimmed} sequences from the BEHAVE test set. We keep the original sequence lengths to stress-test \emph{generalization} and \emph{long-horizon stability}---a challenging regime in which body- and object-IMUs inevitably accumulate drift. Each column corresponds to a method (DIP*, TIP*, TransPose*, GlobalPose*, IMUHOI, and GT), and rows show different interaction sequences ordered from \emph{earlier} to \emph{later} in time (arrow in the GT column).

Across the first three rows (typical daily interactions), the extended baselines progressively lose the hand--object alignment: the object gradually \emph{slides} away from the hand, contact is intermittently broken, and the relative human--object placement becomes inconsistent with the scene. In contrast, our IMUHOI preserves the grasp configuration and the hand--object distance over time, matching the ground-truth progression.

The \textbf{fourth row} is a particularly \emph{challenging} long-horizon case. Here, methods that rely purely on IMUs for object pose (all baselines) suffer pronounced \emph{global drift}: the object trajectory deviates substantially and the interaction collapses after a long run. Our approach remains stable for the entire sequence, keeping the object consistently attached to the interacting hand(s) and maintaining a plausible human--object relative pose. We attribute this robustness to the proposed \emph{contact-gated fusion}: when confident hand contact is detected, the FK branch anchors the object to the hand; when contact weakens, the IMU branch fills in motion, and the gate mediates smooth transitions. 

Overall, the qualitative trends in Fig.~\ref{fig:qualitative_compare} echo our quantitative gains: on long sequences where IMU drift is unavoidable, IMUHOI suppresses drift and preserves interaction semantics, while the extended HPE baselines eventually lose contact or accumulate large trajectory errors.


% ---------------- Table 3 ----------------
\begin{table}[t]
\centering
\caption{Ablation of our object-translation heads. Numbers are lower-is-better. Best in \textbf{bold}.}
\label{tab:ablation_heads}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.05}
\scriptsize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{OMOMO}
& \multicolumn{2}{c}{$IMHD^{2}$}
& \multicolumn{2}{c}{BEHAVE} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
\textbf{Methods} 
& Obj Err & HOI Err
& Obj Err & HOI Err
& Obj Err & HOI Err \\
\midrule
Our Method -- FK
& 31.06 & 32.51
& 61.58 & 57.64
& 23.68 & \textbf{24.58} \\
Our Method -- IMU Only
& 11.52 & 18.07
& 68.59 & 72.58
& 22.99 & 28.03 \\
\textbf{Our Method -- Fusion}
& \textbf{11.31} & \textbf{17.44}
& \textbf{43.97} & \textbf{43.39}
& \textbf{20.90} & 25.74 \\
\bottomrule
\end{tabular}%
}
\vspace{-0.5em}
\end{table}
% ---------------- Table 4 ----------------
\begin{table}[t]
\centering
\caption{Fusion on off-the-shelf IMU HPE backbones. Numbers are lower-is-better. Best in \textbf{bold}.}
\label{tab:plug_backbone}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.06}
\scriptsize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{OMOMO}
& \multicolumn{2}{c}{$IMHD^{2}$}
& \multicolumn{2}{c}{BEHAVE} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
\textbf{Methods}
& Obj Err & HOI Err
& Obj Err & HOI Err
& Obj Err & HOI Err \\
\midrule
DIP*                      & 25.84 & 26.79 & 90.37 & 93.09 & 38.91 & 39.31 \\
DIP* \;--\; Fusion        & \textbf{13.95} & \textbf{15.59} & \textbf{46.11} & \textbf{50.64} & \textbf{22.41} & \textbf{24.96} \\
\midrule
Transpose*                & 32.54 & 32.73 & 90.37 & 90.61 & 40.39 & 40.40 \\
Transpose* \;--\; Fusion  & \textbf{14.03} & \textbf{29.52} & \textbf{47.16} & \textbf{52.55} & \textbf{22.44} & \textbf{35.07} \\
\midrule
GlobalPose*               & 39.34 & 39.51 & 101.27 & 102.03 & 40.14 & 40.21 \\
GlobalPose* \;--\; Fusion & \textbf{14.22} & \textbf{20.60} & \textbf{46.70} & \textbf{53.69} & \textbf{22.69} & \textbf{27.98} \\
\bottomrule
\end{tabular}%
}
\vspace{-0.5em}
\end{table}

% ---------------- Fig 4 ----------------
\begin{figure}[t]
    \centering
    % 调整宽度比例 0.95\linewidth 或 1.0\linewidth 都可以
    \includegraphics[width=1.0\linewidth]{figs/table3_vis.pdf}
    \vspace{-1.5em}
    \caption{
        TODO
    }
    \label{fig:curve_hoi_error}
    \vspace{-1em} % 调整与正文间距
\end{figure}

\subsection{Ablation Studies}
\label{subsec:ablation}
\paragraph{Effectiveness of the object-translation heads.} %这个标题要改改，不知所云，后面一起想想
Table~\ref{tab:ablation_heads} compares three variants: \emph{FK only}, \emph{IMU only}, and our \emph{Fusion}. 
Fusion consistently yields the best Obj Err on all datasets and the best (or near-best) HOI Err on two out of three datasets.
Concretely, relative to the stronger single head on each dataset, Fusion reduces
Obj Err by 0.21 (1.8\%) and HOI Err by 0.63 (3.5\%) on OMOMO (vs.\ IMU-only);
by a much larger margin on the small $IMHD^{2}$ set, Obj Err drops 17.61 (28.6\%) and HOI Err drops 14.25 (24.7\%) (vs.\ FK-only);
and on BEHAVE our Fusion improves Obj Err by 2.09 (9.1\%) over IMU-only while achieving the second-best HOI Err, within 4.7\% of FK-only.
These gains indicate that neither IMU-only (accurate but drifting) nor FK-only (anchored but locally biased) suffices alone; combining them under contact gating is crucial for robust object estimation and interaction fidelity.

\paragraph{Error–time curves and crossover behavior.}
To further probe the dynamics, we plot cumulative errors for the three heads and mark four reference times \textbf{A–D}; the right-hand panels show the corresponding visualizations (each with four people–object pairs).
At \textbf{A} (short horizon), the \emph{IMU-only} branch exhibits the lowest error—its raw inertial integration excels at capturing high-frequency, short-range motion with high \emph{instantaneous} accuracy.
By \textbf{B} (longer horizon), \emph{FK-only} becomes preferable: anchoring the object to the hand through kinematics/contact prevents early drift, so its curve grows more slowly than IMU-only.
At \textbf{C}, our \emph{Fusion} overtakes both—contact-gated routing leverages FK when hand–object contact is confident (to avoid slippage) while still injecting IMU cues for short-term precision, producing a curve below both single heads.
Finally, by \textbf{D} (sequence end, $\approx\!120$\,s), \emph{neither} IMU-only \emph{nor} FK-only preserves attachment—the object has clearly separated from the hand on both, which we attribute to accumulated errors caused by occasional contact-label inaccuracies that shift the interaction point and compound over time. In contrast, \emph{Fusion} remains stable and attached by reweighting branches when contact confidence changes and by enforcing kinematic–inertial consistency, explaining the large long-horizon advantage observed in Table~\ref{tab:ablation_heads}.

\paragraph{Backbone-agnostic plug-in study.}
Because the human module in our pipeline is replaceable, we compare simply augmenting each HPE backbone with an object head against plugging the same backbone into our contact-gated Fusion (Table~\ref{tab:plug_backbone}). Across all datasets, the Fusion plug-in yields clear improvements on object-centric metrics over the dimension-augmented baselines. Especially for GlobalPose* on the $IMHD^{2}$ dataset, Obj Err is reduced 54.57 (53.9\%) and HOI Err is reduced 48.34 (47.4\%), highlighting that our plug-and-play fusion substantially upgrades existing HPE models for HOI.


